SHRINK: Data Compression by Semantic Extraction and Residuals Encoding

The distributed data infrastructure in Internet of Things (IoT) ecosystems requires efficient data-series compression methods, along with the ability to feed different accuracy demands. However, the compression performance of existing compression methods degrades sharply when calling for ultra-accurate data recovery. In this paper, we introduce SHRINK, a novel highly accurate data compression method that offers a higher compression ratio and also lower runtime than prior compressors. SHRINK extracts data semantics in the form of linear segments to construct a compact knowledge base, using a dynamic error threshold that it adapts to data characteristics. Then, it captures the remaining data details as residuals to support lossy compression at diverse resolutions as well as lossless compression. As SHRINK identifies repeated semantics, its compression ratio increases with data size. Our experimental evaluation demonstrates that SHRINK outperforms state-of-art methods with an up to threefold improvement in compression ratio.

==> figures/algorithms/BaseConstruction.tex <==
% \begin{algorithm}
% \caption{Base Construction}
% \begin{algorithmic}[1]
% \State \textbf{Input:} $\semantic$ 
% \State \textbf{Output:} $B_x^{\epsilon_{b}}$
% \Function{BaseConstruction}{$Semantics$}
%     \State $Root \gets PriorityQueue()$ 
%      \For{$c$ in $\semantic$ }
%         \State $Root.append($c$)$
%       \EndFor
%       \State $B_x^{\epsilon_{b}} \gets Merge(Root)$
%     \State \textbf{return} $B_x^{\epsilon_{b}}$
% \EndFunction
% \end{algorithmic}
% \label{alg:BaseConstruction}
% \end{algorithm}

\begin{algorithm}
\caption{Base Construction}
\begin{algorithmic}[1]
\State \textbf{Input:} $\semantic$ 						 \label{BC:line:1}
\State \textbf{Output:} $B_x^{\epsilon_{b}}$			 \label{BC:line:2}
\Function{BaseConstruction}{$\semantic$}                 \label{BC:line:3}
    \State $Root \gets PriorityQueue()$                   \label{BC:line:4}
     \For{$c$ in $\semantic$ }                           \label{BC:line:5}
        \State $Root.insert($c$)$    \Comment{order by $\origin$ and $\Span^{-}$}                                      \label{BC:line:6}
      \EndFor                                            \label{BC:line:7}
      \For{$\origin_i$ in $Root$ }                           \label{BC:line:8}
            \State $subbase \gets [\Span^{-}=-\infty,\Span^{+}=\infty,t=NULL]$ \label{BC:line:9}
            \For{$\Span_j$ in $\origin_i$ } \label{BC:line:10}
                    \If{$\Span_j^{-}\leq subbase.\Span^{+}$ \textbf{and} $\Span_j^{+}\geq subbase.\Span^{-}$}  \label{BC:line:11}
                            \State $subbase.\Span^{-} \gets max(\Span_j^{-}, subbase.\Span^{-})$ \label{BC:line:12}
                            \State $subbase.\Span^{+} \gets min(\Span_j^{+}, subbase.\Span^{+})$ \label{BC:line:13}
                            \State $subbase.t.append(t_j) $ \label{BC:line:14}
                        \Else $ $ \label{BC:line:15}
                            \State $B_x^{\epsilon_{b}}.insert([\origin_i,subbase])$  \label{BC:line:16}
                            \State $subbase \gets [\Span^{-}=\Span_j^{-},\Span^{+}=\Span_j^{+},t=t_j]$ \label{BC:line:17}
                        \EndIf\label{BC:line:18}
            \EndFor \label{BC:line:19}
      \EndFor \label{BC:line:20}                                           
     \State \textbf{return} $B_x^{\epsilon_{b}}$          \label{BC:line:21}
\EndFunction
\end{algorithmic}
\label{alg:BaseConstruction}
\end{algorithm}

==> figures/algorithms/CandidateLine.tex <==
% \begin{algorithm}
% \caption{Candidate Line Selection}
% \begin{algorithmic}[1]
% \State \textbf{Input:}  $\Span^{-}$, $\Span^{+}$
% \State \textbf{Output:} Slope $\mu$ of candidate line
% \Function{OptimizedSlope}{$\Span^{-}$, $\Span^{+}$}
%     \State $lead_1 \gets \Call{ExtractIntegerPart}{\Span^{-}}$
%     \State $lead_2 \gets \Call{ExtractIntegerPart}{\Span^{+}}$
%     \If{$lead_1 \neq lead_2$}
%         \State \Return $\Call{Round}{(\Span^{-} + \Span^{+}) / 2, 1}$
%     \EndIf
%     \State $tail_1 \gets \Call{ExtractDecimalPart}{\Span^{-}}$
%     \State $tail_2 \gets \Call{ExtractDecimalPart}{\Span^{+}}$
%     \State $tail \gets \Call{LongestCommonPrefix}{tail_1, tail_2}$
%     \State $\mu \gets \Call{Concatenate}{lead_1, '.', tail}$
%     \State \textbf{return} $\mu$
% \EndFunction
% \end{algorithmic}
% \label{alg:CandidateLine}
% \end{algorithm}


\begin{algorithm}
\caption{Candidate Line Selection}
\begin{algorithmic}[1]
\State \textbf{Input:}  $\Span^{-}$, $\Span^{+}$						\label{CL:line:1}
\State \textbf{Output:} Slope $\mu$ of candidate line					 \label{CL:line:2}
\Function{OptimizedSlope}{$\Span^{-}$, $\Span^{+}$}                      \label{CL:line:3}
    \State $lead_1 \gets \Call{ExtractIntegerPart}{\Span^{-}}$           \label{CL:line:4}
    \State $lead_2 \gets \Call{ExtractIntegerPart}{\Span^{+}}$           \label{CL:line:5}
    \If{$lead_1 \neq lead_2$}                                            \label{CL:line:6}
        \State \Return $\Call{Round}{(\Span^{-} + \Span^{+}) / 2, 1}$    \label{CL:line:7}
    \EndIf                                                               \label{CL:line:8}
    \State $tail_1 \gets \Call{ExtractDecimalPart}{\Span^{-}}$           \label{CL:line:9}
    \State $tail_2 \gets \Call{ExtractDecimalPart}{\Span^{+}}$           \label{CL:line:10}
    \State $tail \gets \Call{LongestCommonPrefix}{tail_1, tail_2}$       \label{CL:line:11}
    \State $\mu \gets \Call{Concatenate}{lead_1, '.', tail}$             \label{CL:line:12}
    \State \textbf{return} $\mu$                                         \label{CL:line:13}
\EndFunction
\end{algorithmic}
\label{alg:CandidateLine}
\end{algorithm}


==> figures/algorithms/ResidualEncoding.tex <==
% \begin{algorithm}
% \caption{Residuals Encoding}
% \label{alg:residualencode}
% \begin{algorithmic}[1]
% \State \textbf{Input:}  $B_x^{\epsilon_{b}}$
% \State \textbf{Output:} $r_x^{\epsilon_{r}}$
% \Function{EncodeResiduals}{$B_x^{\epsilon_{b}}$}

%         \For{each $b$ in $B_x^{\epsilon_{b}}$} 
%             \State $\Span_b \gets OptimizedSlope(\Span^{-}_b, \Span^{+}_b)$
%             % \State $B \gets Decompose(B_x^{\epsilon_{b}})$
%             \State $r \gets X - B_x^{\epsilon_{b}}$
%             \State $\hat{r} \gets Quantiz(r)$
%             \State $R \gets R \cup \{\hat{r} \}$
%         \EndFor
%         \State $r_x^{\epsilon_{r}}  \gets EntropyCoding(R)$
        
%     \State \textbf{return} $r_x^{\epsilon_{r}}$
% \EndFunction
% \end{algorithmic}
% \label{alg:ResidualEncoding}
% \end{algorithm}


\begin{algorithm}
\caption{Residuals Encoding}
\label{alg:residualencode}
\begin{algorithmic}[1]
\State \textbf{Input:}  $B_x^{\epsilon_{b}}, \epsilon_r	$							\label{RE:line:1}
\State \textbf{Output:} $R_x^{\epsilon_{r}}$								 \label{RE:line:2}
\Function{EncodeResiduals}{$B_x^{\epsilon_{b}}, \epsilon_r$}                             \label{RE:line:3}
		\State $R \gets [ ]$																	 \label{RE:line:4}
        \For{each $b_i$ in $B_x^{\epsilon_{b}}$}                               \label{RE:line:5}
            \State $\Span_{b_{i}} \gets OptimizedSlope(\Span^{-}_{b_{i}}, \Span^{+}_{b_{i}})$  \label{RE:line:6}
            % \State $B \gets Decompose(B_x^{\epsilon_{b}})$                 \label{RE:line:7}
            \State $r_{b_{i}} \gets X_{b_{i}} - sketch(b_i, \Span_{b_{i}})$                          \label{RE:line:7}
            \State $R.append(r_{b_{i}})$                          \label{RE:line:8}
        \EndFor                                             \label{RE:line:9}
            \State $R_x^{\epsilon_{r}} \gets Quantize(R, \epsilon_{r})$                                \label{RE:line:10}
    \State \textbf{return} $R_x^{\epsilon_{r}}$                              \label{RE:line:11}
\EndFunction
\end{algorithmic}
\label{alg:ResidualEncoding}
\end{algorithm}

==> figures/algorithms/SemanticsExtraction.tex <==
\begin{algorithm}
    \caption{Semantics Extraction}
    \begin{algorithmic}[1]
    \State \textbf{Input:} Data series $X$																				\label{se:line:1}
    \State \textbf{Output:} Semantics  $\semantic$                                                                      \label{se:line:2}
    \Function{SemanticsExtraction}{$X$}                                                                                 \label{se:line:3}
    \State $\semantic \gets []$                                                                                         \label{se:line:4}
    \State $\Span^{+} \gets \infty$                                                                                     \label{se:line:5}
    \State $\Span^{-} \gets -\infty$                                                                                    \label{se:line:6}
    \State $\origin_0 \gets DIVISION({0})$                                                                                \label{se:line:7}
    \For{$(t_i, v_i)$ in $X$}                                                                                                  \label{se:line:8}

        %\If{$v_0<v_i-\hat{\epsilon}_{b}-\Span^{+}(t_i-t_0)$ {or} $v_0>v_i+\hat{\epsilon}_{b}-\Span^{+}(t_i-t_0)$}    
        %\If{$v_0 < v_i - \hat{\epsilon}_{b} - \Span^{+}(t_i - t_0)$ \textbf{or} $v_0 > v_i + \hat{\epsilon}_{b}-\Span^{+}(t_i - t_0)$}
        \If{$\origin_0 < v_i - \hat{\epsilon}_{b} - \Span^{+}\Delta t $ \textbf{or} $\origin_0 > v_i + \hat{\epsilon}_{b} - \Span^{+}\Delta t$}
        \label{se:line:9}
            \State $\semantic.insert([\origin_0, \Span^{-}, \Span^{+},  t_0])$                                       \label{se:line:10}
            \State $\origin_i \gets DIVISION({i})$                                       
            \label{se:line:11}
            \State $(t_0, \origin_0) \gets (t_i, \origin_i)$
            \label{se:line:12}
            \State $\Span^{+} \gets \infty$                                                                             \label{se:line:13}
            \State $\Span^{-} \gets -\infty$                                                                            \label{se:line:14}
        \Else $ $ 
            \State $\Span^{+}  \gets min(\Span^{+}, \frac{v_i+\hat{\epsilon}_{b}-\origin_0}{\Delta t})$  
             \label{se:line:15}
            \State $\Span^{-}  \gets max(\Span^{-},\frac{v_i-\hat{\epsilon}_{b}-\origin_0}{\Delta t})$                                                      \label{se:line:16}
        \EndIf                                                                                                          \label{se:line:17}
    \EndFor                                                                                                             \label{se:line:18}
    \State \textbf{return} $\semantic$                                                                                  \label{se:line:19}
    \EndFunction
    \end{algorithmic}
    \label{alg:SemanticsExtraction}
\end{algorithm}

==> figures/algorithms/phase.tex <==
\begin{algorithm}[!h]																			
    \caption{Phases Division}
    \begin{algorithmic}[1]
    \State \textbf{Input:}  Index of point $j$																				\label{phase:line:1}
    \State \textbf{Output:} Origin of a new cone $\origin$                                                                  \label{phase:line:2}
    \Function{Division}{$j$}                                                                                                \label{phase:line:3}
        \State $L \gets \lambda \cdot n \cdot \epsilon_{b} $                                                                \label{phase:line:4}
        \State $Interval \gets X[j : j+L] $                                                                                 \label{phase:line:5}
        \State $\Delta \gets max - min$                                                                                     \label{phase:line:6}
        \For{ each $v$ in the Interval}                  \label{phase:line:7}
            \State $update(v_{max}, v_{min})$   \label{phase:line:8}
        \EndFor                                                  \label{phase:line:9}
        \State $\Delta_i \gets v_{max} - v_{min}$ \Comment{i is the index of interval}                                      \label{phase:line:10}
        \State $\beta_i \gets \Delta_i/\Delta$                                                                                \label{phase:line:11}
        \State $\hat{\epsilon}_b \gets \epsilon_{b} \cdot e^{(2/3 - \beta_i)}$ 
            \label{phase:line:12}
        \State $ \origin \gets \left\lfloor {v_i}\cdot \frac{1}{\hat{\epsilon}_b} \right\rfloor  \cdot {\hat{\epsilon}_b}$      \label{phase:line:13}
        \State \textbf{return}  $\origin$                                                                                   \label{phase:line:14}
    \EndFunction
    \end{algorithmic}\label{alg:phase}
\end{algorithm}

==> figures/algorithms/workflow.tex <==
\begin{algorithm}[!h]
\caption{Overall workflow of \name}\label{alg:workflow}
    \begin{algorithmic}[1]
        \State \textbf{Input:}  $X$, $E = $ \{$\epsilon_1$, $\epsilon_2$,...,$\epsilon_n$ \}, $\epsilon_{b}$ \label{lst:line:1}
        \State \textbf{Output:}  $C_x$                                                      \label{lst:line:2}
        \State $C_x \gets []$                                                                                  \label{lst:line:3}
        \State $ \mathscr{S} \gets \text{SemanticExtraction(X)}$ \Comment{\autoref{sec:Semantics}}              \label{lst:line:4}
        \State $ B_x^{\epsilon_{b}} \gets \text{BaseConstruction($\mathscr{S}$)}$ \Comment{\autoref{sec:Base}}  \label{lst:line:5}
        \State $\hat{B}_x^{\epsilon_{b}} \gets EntropyCoding(B_x^{\epsilon_{b}})$ \Comment{optional}                           \label{lst:line:6}
        \State $C_x.insert(\hat{B}_x^{\epsilon_{b}}) $ 
            \label{lst:line:7}
        \For{ $\epsilon_i$ in $E$}                                                                                                \label{lst:line:8}
                \If{$\epsilon_i \geq \hat{\epsilon}_b$}                                                                         \label{lst:line:9}
                    \State $C_x^i \gets NULL$
                       \label{lst:line:10}  
                \Else $ $ \label{lst:line:11}
                    \State $R_x^{\epsilon_{i}} \gets \text{EncodeResidual}(r, \epsilon_i)$ \Comment{\autoref{sec:residual}}\label{lst:line:12}
                    \State $C_x^i \gets EntropyCoding(R_x^{\epsilon_{i}})$
                    \label{lst:line:13}
                \EndIf                                                                                               \label{lst:line:14}
                \State $C_x.insert(C_x^i) $                                                                               \label{lst:line:15}
                % \State $C_x \gets C_x \cup \{B_x^{\epsilon_{b}} \oplus  R_x^{\epsilon_{i}}\}$                           \label{lst:line:13}
        \EndFor                                                                                                         \label{lst:line:16}
        \State \textbf{return} $C_x$                                                                                     \label{lst:line:17}
    \end{algorithmic}
\end{algorithm}


==> sections/03.5.proofs.tex <==
\subsection{Proof of Correctness and Complexity}\label{sec:complexity}

Here we provide a proof of correctness of \name and discuss its complexity. To simplify the complexity analysis, we do not consider the process of entropy coding.

\setcounter{theorem}{0}
\begin{theorem}
The reconstructed data from the compressed form~$C_x$ achieve accuracy loss below the error threshold~$\epsilon$.
\end{theorem}
\begin{proof}
We consider two extreme cases. For the case that the compressed data~$C_x$ consists only of base. Then, if we set the statement in Line~4 of Algorithm~\ref{alg:phase} as~$L \gets \frac{1}{\epsilon_{b}} \cdot n \cdot \epsilon_{b}$, \name is equivalent to \simpiece~\cite{kitsios2023sim} with error bound~$\epsilon_b$. Therefore, the approximation by \name is the same of that by \simpiece, and the reconstructed data by both are within error threshold~$\epsilon_b$. In case the compressed data comprises base and residuals, i.e.,~$C_x = B_x^{\epsilon_{b}} \oplus R_x^{\epsilon_r}$, the achieved error guarantee is within~$\hat{\epsilon}_b$. Each residual value~$r_i$ is in $[-\hat{\epsilon}_b, \hat{\epsilon}_b]$, while the quantization error of residuals is within~$\epsilon_r \leq \epsilon$. The final reconstructed data accuracy depends solely on the residual quantization with~$\epsilon_r \leq \epsilon$, hence it is within the target maximum absolute error threshold~$\epsilon$.
\end{proof}

\begin{theorem}
Given a data series of length~$n$, the computational complexity of \name is~$\mathcal{O}(n) + \mathcal{O}(q \log q)$, where~$q$ is the number of cones created.
\end{theorem}

\begin{proof}
The time complexity of \simpiece is~$T_\textit{SIMPIECE} = \mathcal{O}(n) +  \mathcal{O}(m \log m)$, where~$m$ is the maximum number of line segments created. Assume an interval of length~$L$ and~$q$ cones and~$k$ sub-bases. Then, the time complexity of \name is determined by three processes: (i) the time to extract semantics~$\semantic$, including~$\Delta$ in~$\mathcal{O}(n)$, calculating~$\Delta_i$ in~$\mathcal{O}(L)$, and creating cones in~$\mathcal{O}(L)$. Thus,~$T_1 = \mathcal{O}(n) + \mathcal{O}(kL) + \mathcal{O}(L) = \mathcal{O}(n)$; (ii) the time to construct base is dominated by the cost of sorting cones; in the worst case we only have one phase with all cones, hence the time complexity is~$T_2 = \mathcal{O}(q \log q)$; (iii) the time complexity to encode residuals is~$T_3 = \mathcal{O}(n)$, as we process residual values sequentially. Thus, the overall time complexity is~$T_\textit{SHRINK} = \mathcal{O}(n) + \mathcal{O}(q \log q)$. As \name uses a coarse-grained error threshold~$\epsilon_b$, it produces fewer cones than \simpiece, hence~$q \leq m$, therefore the time complexity of \name is in the same order as that of \simpiece, while \name accelerates compression in practice.
\end{proof}



==> sections/04.1.benchmarks.tex <==
\subsection{Comparison benchmarks}

\name provides error-bounded compression that captures important features, i.e., semantics, and can dynamically adjust error resolution. Note that \name provides lossless compression when error-bound is set to 0. Hence, we compare it to the following existing lossless and lossy compression methods.

\subsubsection{Lossless benchmarks}

\begin{itemize}
\item \textbf{Bzip2}\footnote{https://docs.python.org/3/library/bz2.html}: \pk{a lossless compression method that uses the Burrows-Wheeler algorithm and Huffman coding, well-known for its high compression ratio and often used for compressing files~\cite{bzip2site}; Bzip2 typically produces smaller files than Gzip.}
\item \textbf{Gzip}\footnote{https://docs.python.org/3/library/gzip.html}: \pk{a lossless compression method that first compresses the designated file using a modified version of the LZ77 algorithm, and then applies additional compression through Huffman coding~\cite{gzipsite}, choosing between static or dynamic Huffman encoding based on the circumstances.}
\item \textbf{TRC}\footnote{https://github.com/powturbo/Turbo-Range-Coder}: \pk{a lossless compression scheme that operates on the principles of arithmetic coding, dividing the input data stream into several blocks and compressing these blocks in parallel using multiple arithmetic encoders~\cite{turboRangeCoder}; it takes full advantage of parallel processing to accelerate the compression process, while maintaining data integrity. We also use TRC for the final entropy coding process in \name.}
\item \textbf{Gorilla}\footnote{https://pypi.org/project/gorillacompression}: \pks{a lossless compression method designed specifically for time-series data. It employs delta-of-delta encoding for efficient timestamp compression and XOR encoding to minimize storage via leading and trailing zero suppression.}
\item \textbf{GD}: \pks{a novel Generalized Deduplication-based compression algorithm designed to enhance both compression performance and allow direct analytics on compressed data. We used the latest version, \ggd~\cite{hurst2024greedygd}.}
\end{itemize}

\subsubsection{Lossy benchmarks} 

\begin{itemize}
\item \textbf{\simpiece}\footnote{https://github.com/xkitsios/sim-piece}: \pk{the state-of-the-art method based on piecewise linear approximation (PLA) with maximum error guarantees~\cite{kitsios2023sim}, which groups line segments to represent them jointly, hence achieves higher compression ratio than traditional PLA algorithms~\cite{luo2015piecewise, lazaridis2003capturing, elmeleegy2009online}. For the sake of a fair comparison, we apply TRC to perform entropy encoding in \simpiece too.}
\item \textbf{APCA} (Adaptive Piecewise Constant Approximation): a method that yields a set of constant-value segments of varying lengths~\cite{keogh2001locally}, adaptively tuning segment size to enforce an error bound; the implementation, kindly provided by the authors of~\cite{barbarioli2023hierarchical}.
\item \textbf{HIRE}\footnote{https://github.com/gmersy/HIRE}: \pk{designed to address multi-resolution compression problems~\cite{barbarioli2023hierarchical}, HIRE divides a dataset to multiple blocks sizes as powers of~2. Similarly to \name, it allows for an encoding that can be decompressed at multiple resolutions. HIRE outperforms multiple existing compression methods in low precision.}
\item \textbf{LFZip}\footnote{https://github.com/shubhamchandak94/LFZip/tree/master}: \pk{a method based on a prediction-quantization-entropy coder framework, benefiting from improved prediction using simple neural networks~\cite{chandak2020lfzip}.}
\end{itemize}

==> sections/04.5.general.tex <==
\input{texfigures/multiresolution}

\subsection{\pks{Comparison to general-purpose compression}}

We evaluate the performance of SHRINK against two general-purpose lossy compression methods, HIRE and LFZip, using error resolution levels ranging from 1e-2 to~1e-5 on a logarithmic scale. \gy{This selection ensures a comprehensive evaluation across broad error thresholds, reflecting the stringent precision requirements and varied application scenarios of general-purpose methods.} For WindSpeed and WindDirection, the error still ranges from~1e-2 to~1e-3 due to limited decimal places. We set~$\epsilon_b$ as~15\% of the data range as the compression performance is the main goal for general purpose compression, rendering it unnecessary to set a small {$\epsilon_b$}. \autoref{fig:multiresolution} presents our results, in which the dashed line indicates the lossless compression ratio achieved by \name. Our results demonstrate that SHRINK consistently outperforms HIRE and LFZip across nearly all datasets and error thresholds, achieving higher compression ratios while maintaining data accuracy, particularly at stringent error thresholds,~$\epsilon \le 10^{-3}$.

%, yet deteriorate rapidly as precision requirements rise. Here, we evaluate \name against two general-purpose lossy compression methods, HIRE and LFZip. \autoref{fig:multiresolution} presents our results, in which the dashed line indicates the lossless compression ratio achieved by \name. The error resolution~$\epsilon$ ranges from~1e-2 to~1e-5 on a logarithmic scale. For WindSpeed and WindDirection data, the error ranges from~1e-2 to~1e-3 due to limited decimal places. We set~$\epsilon_b$ as~50\% of the data range as the compression performance is the main goal for general purpose compression, rendering it unnecessary to set a small {$\epsilon_b$}. Notably, \name outperforms HIRE and LFZip in nearly all data series, especially at strict~$\epsilon$ thresholds. These results indicate a superior ability on behalf of \name to balance data accuracy with compression.

It is worth mentioning that on the FaceFour, MoteStrain, ECG, and Cricket datasets, the lossless compression ratio of \name surpasses even the lossy compression ratios of HIRE and LFZip at~$\epsilon$ values less than~$10^{-4}$. \pks{This outcome indicates that these compression methods fail to provide competent compression enabling highly accurate data recovery}. The superior performance of \name in this context suggests its applicability in real-world scenarios that prioritize accuracy. Many practical applications, such as medical (e.g., ECG) data analysis and seismic data analysis, demand high-precision data to maintain result integrity and reliability. As \name maintains a high compression ratio without compromising data accuracy, it would be suitable for these high-stakes applications.

\gy{The selection of error thresholds differs from those in~\ref{sec:Semantics} due to the distinct objectives and natures of the compared methods. Lossy piecewise segment compression methods (\simpiece and APCA), specifically piecewise linear approximation, aim to capture meaningful structure or mine datasets based on a representation of data~\cite{keogh2001online}. Thus, different error thresholds are significant as traditional PLA methods do not adjust their error thresholds adaptively to capture more meaningful structures or semantics of data. Therefore, we use a more detailed error resolution rather than a broader one for PLA methods. On the other hand, general-purpose compression methods are designed to perform efficiently across a broader spectrum of error tolerances to achieve higher compression ratios. The broader error resolution range selected for this section ensures that the evaluation reflects typical use cases for these versatile methods while maintaining rigorous precision. Thus, we do not need to use as fine-grained a comparison for general-purpose methods. However, SHRINK achieves a balance between them, as it can not only adaptively capture meaningful semantics but also adjust errors in a broader range to improve its performance.}

==> sections/04.7.edge.tex <==
\subsection{Evaluation of Edge}

%previous versio: NVIDIA TU102~GPU, 31~processors, and~125GB RAM
To evaluate the workflow in Edge, we simulated an application that requests the Pressure data set stored at an Edge server equipped with AMD Ryzen 7 PRO 6850U  with Radeon Graphics (16 cores) and 16GB RAM, at ten different error resolutions, i.e.,~\{0.01, 0.0075, 0.005, 0.0025, 0.001, 0.00075, 0.0005, 0.00025, 0.0001, 0.00001\}; this array of error resolutions covers most real-world compression usages. The requests arrive in a random order. We evaluate \name compared to three lossy methods, $\simpiece$, HIRE and LFZip, and a lossless method, GZip.

We evaluate the following three measures:
\begin{itemize}
\item Max Local Storage (MLS): the maximum amount of data stored on edge locally.
\item Average Transferred Size (ATS): the average data size transferred from the edge to the remote server over all requests.
\item Average Processing Latency (APL): the average time needed for encoding per retrieval request, excluding data transfer.
\end{itemize}

\input{tables/Edge}

Table~\ref{tab:Edge} presents our simulation results. \name significantly reduces the local storage while satisfying all the requests, as it only needs to store the knowledge base and the residuals at the stringent error resolution of~$0.00001$. Besides, \name does not need to transfer all the required data at different resolutions. It only needs to transmit one knowledge base and different residuals, thus achieves significantly low ATS. In a real scenario with many applications consuming the data, the performance will be further increased. While \name needs more processing latency than HIRE, it is still competitive to others, especially \simpiece and lossless compression, enables more efficient use of storage and reduces the size of data transfer. Thus, \name attains comparable latency to the state-of-the-art compression framework, HIRE, designed for multiresolution compression in Edge environments, and considerably reduces data footprint and transfer size. Meanwhile, the lossless method, GZip, always stores and transfers the data in lossless format, unable to leverage the lower resolutions to reduce transferred data size.

%\gy{Table~\ref{tab:Edge} presents evaluation results. \name significantly reduced the local storage to satisfy all the ten requests. The reason is that the compression performance \name does not degrade with lower error threshold, unlike the lossy baselines. Compared to GZip, \name keeps the advantage of the lossy method, gaining a super high compression ratio. Regarding ATS, we do not need to transfer all the required data with different resolutions. In fact, it only has a minor overhead over transmitting one knowledge base and different residuals and thus achieves significantly low ATS. In the real scenario, there are many applications consuming the data, so it is expected that our performance will be increased again. While \name does need more processing latency than HIRE, it is still competitive to others and is significantly smaller than \simpiece and lossless compression. We believe there exists a tradeoff. Edge devices have limited storage, and \name enables more efficient use of local storage. Additionally, network transfers are a significant factor in energy consumption, which \name addresses by substantially reducing transfer size. In other words, we attain comparable latencies to the state-of-the-art compression framework HIRE, which is designed for multiresolution compression in Edge environments, but we can considerably reduce the data footprint and transfer size.}

==> sections/06.related.tex <==
\section{Related Work}

% online algorithm not relevant to us.
%Keogh et al.~\cite{keogh2001online} proposed an online algorithm for time series segmentation, surpassing existing piecewise linear approximation (PLA) techniques in approximation quality and computational efficiency.
\noindent \textbf{Piecewise approximations.} \pk{A first effort to provide semantics-oriented data approximation was Adaptive Piecewise Constant Approximation (APCA)~\cite{keogh2001locally}, an indexable dimensionality reduction technique for time series databases. More powerfully, Swing and Slide~\cite{elmeleegy2009online} produce connected as well as disconnected piecewise linear segments of variable length with error guarantees. Mixed-PLA~\cite{luo2015piecewise} combines the advantages of joint and disjoint linear segments and optimizes the size of its representation by dynamic programming based on geometric properties. \simpiece is the state-of-the-art linear-segment-based compression approach; it builds a minimum number of groups that exploits similarities among line segments~\cite{kitsios2023sim} to offer space savings.}

\noindent \textbf{Generalized Deduplication (GD)} \pk{is a lossless compression algorithm for IoT data, which clusters similar blocks of bits into bases and stores the remaining bits as deviations~\cite{vestergaard2020randomly}. Unlike data-level compression methods, GD captures bit-level patterns and confers efficient random access capabilities and high compression performance, even on small data blocks. \ggd is a more recent GD variant which offers reliable and efficient data analytics along with higher compression and lower runtime than prior GD compressors~\cite{hurst2024greedygd}. The base in a GD compressor is usable in downstream tasks. For example, GLEAN~\cite{hurst2022glean} applies GD at edge servers to deliver end-to-end lossless data compression and high-quality edge-based analytics in the IoT, thereby addressing challenges in data transmission, storage, and analytics. \name is also inspired by GD-based methods that demonstrate compressed data can be directly utilized to support downstream tasks. However, whereas previous works focused on bit-level patterns, \name combines data-level and bit-level patterns, hence differs from previous GD-based methods.}

\noindent \textbf{Other compression methods.} \pks{Several other compression methods for data series have been proposed. Gorrila~\cite{pelkonen2015gorilla} employs a bitwise XOR operation between consecutive values to derive a lossless encoding that discards useless bits to reduce storage. Chimp~\cite{liakos2022chimp} addresses the limitations of Gorilla by leveraging the inherent characteristics of floating-point numbers to achieve space savings and faster compression speeds. However, as they forfeit data pattern learning, Gorilla and Chimp underperform general-purpose compression methods in compression ratio. LFZip~\cite{chandak2020lfzip} offers error-bounded lossy compression for floating-point data series, leveraging a prediction-quantization-entropy coder framework that incorporates linear models and neural networks. LFZip improves compression ratios over previous compressors, such as SZ~\cite{di2016fast}. HIRE~\cite{barbarioli2023hierarchical} encodes data across multiple resolutions leveraging a hierarchical residual encoding to facilitate data access at varying levels of granularity. While HIRE achieves a smaller storage footprint than LFZip, as we discussed, its compression performance degrades at high-precision compression levels. Similarly to HIRE, \name also furnishes multi-resolution compression, yet our focus is on high-precision compression.}

\noindent \textbf{Other uses of linear approximations.} \pks{Some other related works construct piecewise-linear approximations in a similar manner, yet for other purposes. SIEVE~\cite{tong2023sieve} is a learning-enhanced index that filters out irrelevant data blocks in analytics by capturing data patterns. Likewise, FITing-Tree approximates an index with a bounded error specified at construction time~\cite{galakatos2019fiting}. Both these methods utilize piecewise linear functions to capture patterns in a dataset.}

% Some other traditional works also motivate this work, include Discrete Wavelet Transform ~\cite{karras2005one}, Discrete Fourier Transform ~\cite{hu2016accelerating} and Discrete Cosine Transform~\cite{joshua2016comparison}. Each one has its advantages and disadvantages. Nevertheless, we gain the most from PLA and GD methods.

==> tables/Edge.tex <==
% Please add the following required packages to your document preambl% \usepackage{booktabs}
% use same number of digits for all measurements in the same column
\begin{table}[!h]
\vspace{-1mm}
\centering
\caption{Evaluation on a simulated Edge server.}\label{tab:Edge}
\vspace{-2mm}
\begin{tabular}{@{}lrrr@{}}
\toprule
& \textbf{MLS} & \textbf{ATS} &   \textbf{APL} \\ \midrule
\textbf{SIMPIECE} & 5.728MB      & 4.805MB                  & 13.053s          \\
\textbf{LFZip}    & 21.401MB     & 10.653MB             & 8.130s          \\
\textbf{HIRE}     & 22.041MB     & 9.496MB              & 3.489s          \\
\textbf{GZip}     & 27.056MB     & 27.056MB             & 38.809s       \\
\textbf{SHRINK}   & 1.548MB      & 1.407MB              & 6.185s       \\ \bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}

==> texfigures/CRLossyaverage.tex <==
\begin{figure}[h!]
\vspace{-3mm}
\centering
\includegraphics[width=\linewidth]{figures/CRLossyaverage.pdf}
\vspace{-8mm}
\caption{\gy{Average lossy compression ratio on~9 datasets.}}\label{fig:CRLossyaverage}
\vspace{-3mm}
\end{figure}

==> texfigures/compareForAll.tex <==
\begin{figure}[!t]
%\vspace{-4pt} % 调整垂直空间，负值表示上移标题 % not at top of page
\includegraphics[width=\linewidth]{figures/compareForAll.pdf}
\vspace{-7mm}
\caption{(a)~a data series; (b)~approximation by base; (c)~residual series; (d)~Kernel Density Estimation of residuals.}\label{fig:compareForAll}
\vspace{-2mm}
\end{figure}

==> texfigures/edgeframework.tex <==
\begin{figure}[h!] 
\vspace{-2mm} % 调整垂直空间，负值表示上移标题
\includegraphics[width=\linewidth]{figures/edgeframeworkpdf.pdf}
\vspace{-4mm}
\caption{\pk{Base stored on the edge, residuals on the cloud.}}\label{fig:edgeframework}
\vspace{-2mm}
\end{figure}

==> texfigures/fluctuation.tex <==
\begin{figure}[!h]
\vspace{-1mm}
\centering
\includegraphics[width=\linewidth]{figures/fluctuation.pdf}
\vspace{-5mm}
\caption{\pk{$\hat{\epsilon}_b$ drops as data fluctuates to preserve data patterns.}}\label{fig:fluctuation}
% \vspace{-1mm}
\end{figure}

==> texfigures/intervaltime.tex <==
\begin{figure}[!h]
\centering
\vspace{-2mm}
\includegraphics[width=\linewidth]{figures/intervaltime.pdf}
\vspace{-8mm}
\caption{\pk{Compression latency vs.~$\lambda$.}}
\label{fig:intervaltime}
\vspace{-2mm}
\end{figure}

==> texfigures/sizelossy.tex <==
\begin{figure}[h!]
\centering
\vspace{-2mm}
\includegraphics[width=\linewidth]{figures/sizelossy.pdf}
\vspace{-7mm}
\caption{\pks{Compression ratio at different data sizes.}}\label{fig:sizelossy}
\vspace{-2mm}
\end{figure}
